A Stitch in Time Saves Nine: A Train-Time Regularizing Loss for Improved Neural Network Calibration

Deep Neural Networks ( DNN s) are known to make overconfident mistakes, which makes their use problematic in safety-critical applications. State-of-the-art ( SOTA ) calibration techniques improve on the confidence of predicted labels alone and leave the confidence of non-max classes (e.g. top-2, top-5) uncalibrated. Such calibration is not suitable for label refinement using post-processing. Further, most SOTA techniques learn a few hyper-parameters post-hoc, leaving out the scope for image, or pixel specific calibration. This makes them unsuitable for calibration under domain shift, or for dense prediction tasks like semantic segmentation. In this paper, we argue for intervening at the train time itself, so as to directly produce calibrated DNN models. We propose a novel auxiliary loss function: Multi-class Difference in Confidence and Accuracy ( MDCA ), to achieve the same MDCA can be used in conjunction with other application/task-specific loss functions. We show that training with MDCA leads to better-calibrated models in terms of Expected Calibration Error ( ECE ), and Static Calibration Error ( SCE ) on image classification, and segmentation tasks. We report ECE ( SCE ) score of 0.72 (1.60) on the CIFAR 100 dataset, in comparison to 1.90 (1.71) by the SOTA. Under domain shift, a ResNet-18 model trained on PACS dataset using MDCA gives an average ECE ( SCE ) score of 19.7 (9.7) across all domains, compared to 24.2 (11.8) by the SOTA. For the segmentation task, we report a 2X reduction in calibration error on PASCAL - VOC dataset in comparison to Focal Loss. Finally, MDCA training improves calibration even on imbalanced data, and for natural language classification tasks. We have released the code here: code is available at https://github.com/mdca-loss

==> macros.tex <==
\usepackage{multirow,epsfig,pdflscape,graphicx,amsmath,amssymb}
\usepackage{float}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{textcomp}
\usepackage{mathrsfs}
\usepackage{empheq}
\usepackage{rotating}
	
\usepackage{color, colortbl}
%\definecolor{name}{system}{definition}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\usepackage[table]{xcolor}
%\newcolumntype{litegreen}{>{\columncolor{green}}c}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage[noadjust]{cite}
\usepackage{array, caption, tabularx,  ragged2e,  booktabs}
\usepackage{longtable}
\usepackage{textcomp}
\usepackage{siunitx}
%\usepackage{subfig}
\usepackage{array}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{algpseudocode}
\usepackage{romannum}
\usepackage{graphicx}
\usepackage{xcolor}

\usepackage{times}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{appendix}
\usepackage{etoolbox}
\usepackage{soul}
\usepackage{tabularx}
\usepackage{caption}
\usepackage{subcaption,xspace}

\usepackage[capitalize]{cleveref}

\usepackage[inline]{enumitem}

%\newcommand\figref[1]{Figure~\ref{#1}}
%\newcommand\tabref[1]{Table~\ref{#1}}

%\usepackage{hyperref}

\BeforeBeginEnvironment{appendices}{\clearpage}

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\def\lce{{\mathcal{L}_{\rm CE}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}

\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{remark}{Remarque}

\def\ramya#1{{\color{blue}{\bf [Ramya:} {\it{#1}}{\bf ]}}}
\newcommand\soumya[1]{{\textcolor{red}{[Soumya: #1]}}}
%\newcommand\ram[1]{\textcolor{red}{[Ramya: #1]}}
\newcommand\chetan[1]{\textcolor{purple}{[Chetan: #1]}}
\newcommand\Suban[1]{\textcolor{green}{[Suban: #1]}}

\definecolor{todocolor}{RGB}{200,120,120}
\sethlcolor{todocolor}
\newcommand{\todo}[1]{\textcolor{black}{\hl{#1}}}

%\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\newcommand{\secref}[1]{Sec.~\ref{#1}}
\usepackage{graphicx} 
\usepackage{caption,subcaption}
%\usepackage[showframe]{geometry}

\def\X{{\mathcal{X}}}
\def\Y{{\mathcal{Y}}}
\def\D{{\mathcal{D}}}

\def\dP{{\mathbb{P}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cM{{\mathcal{M}}}
\def\real{{\mathbb{R}}}

\def\etal{{et al.\xspace}}
\def\ood{{OOD\xspace}}
\def\iid{{IID\xspace}}
\def\id{{ID\xspace}}
\def\xt{{\Tilde{x}}}
\def\yt{{\Tilde{y}}}

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{N}{@{}m{0pt}@{}@{}}

% nested enum
\usepackage{enumitem}

\newcommand{\myfirstpara}[1]{\noindent \textbf{#1:}}
\newcommand{\mypara}[1]{\vspace{0.3em} \myfirstpara{#1}}

\newcommand{\multilineC}[1]{\begin{tabular}[b]{@{}c@{}}#1\end{tabular}}
\newcommand{\multilineCB}[1]{\textbf{\multilineC{#1}}}

%\fboxsep=0.2mm%padding thickness
%\fboxrule=0.02pt%border thickness

\graphicspath{{images/}}
\graphicspath{{./imgs/}}



==> sections/buffer.tex <==
%\usepackage{aaai}
%\usepackage{times}
%\usepackage{helvet}
%\usepackage{courier}
%\pdfinfo{
%/Title (Insert Your Title Here)
%/Author (Put All Your Authors Here, Separated by Commas)}
%\setcounter{secnumdepth}{0} 





\begin{figure}[t]
	\centering
	\includegraphics[width =\linewidth]{figs/misclassification_other.pdf}
	%\vspace{-4 mm}
	\caption{Confidence value histogram for \textbf{misclassified} predictions for (a) \texttt{LS}. (b) \texttt{LS+MDCA}, (c) \texttt{FL} and (d) \texttt{FL+MDCA} on the ResNet-20 model trained on SVHN dataset.}
	\label{fig:ConfHist_FLMDCA_vs_FL}
\end{figure}

\mypara{Confidence Values for Incorrect Predictions}
Recall that in our main manuscript, we spoke about our calibration technique reducing the confidence for the mispredictions also. To support the claim, we provided a histogram in the main manuscript for \texttt{MDCA} regularized \texttt{NLL} and \texttt{NLL}, continuing on that, here we provide additional plots that support in  \cref{fig:ConfHist_FLMDCA_vs_FL} that consider the combination of \texttt{MDCA+LS} and its corresponding unregularised \texttt{LS} and \texttt{MDCA+FL} and \texttt{FL} respectively reported on a SVHN dataset.
% \texttt{FL+MDCA} assigns lower confidence to mispredictions than \texttt{FL} considered by itself. 

























\begin{table}[]






\centering
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{c|ccccccc|c}
\toprule
\textbf{Domain}  & \textbf{NLL} & \textbf{Brier Score} & \textbf{LS} & \textbf{Focal Loss} & \textbf{MMCE} & \textbf{DCA} & \textbf{FLSD} & \textbf{FL+MDCA (ours)} \\ \midrule
Clean            & 99.61        & 99.63                & 99.62       & 99.63               & 98.43         & 99.60        & 99.67         & 99.59                   \\
$M_{15}$         & 98.79        & 98.72                & 98.39       & 98.20               & 94.99         & 98.36        & 98.79         & 98.61                   \\
$M_{30}$         & 93.38        & 92.54                & 92.04       & 91.87               & 83.93         & 91.51        & 92.77         & 93.13                   \\
$M_{45}$         & 73.82        & 71.29                & 69.33       & 69.95               & 53.88         & 68.34        & 71.17         & 70.92                   \\
$M_{60}$         & 43.24        & 41.90                & 39.94       & 38.67               & 28.76         & 38.32        & 40.17         & 41.93                   \\
$M_{75}$         & 24.07        & 22.73                & 22.99       & 20.83               & 16.84         & 20.93        & 20.84         & 23.37                   \\ \midrule
\textbf{Average} & 72.15        & 71.14                & 70.39       & 69.86               & 62.81         & 69.51        & 70.57         & 71.26      \\ \bottomrule            
\end{tabular}%
}
\caption{Table comparing Accuracy/Top-1 (\%)  values of our method \texttt{FL+MDCA} with other methods on the Rotated-MNIST dataset trained on a ResNet-20 model.}
\label{tab:mnist-top1-all_methods}
\end{table}



% Test Error % scores
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc|c}
\toprule
\textbf{Dataset}          & \textbf{Model} & \textbf{Cross Entropy} & \textbf{Focal Loss \citeyearpar{ogfocalloss}} & \textbf{LS \citeyearpar{labelsmoothinghelp}} & \textbf{Brier Score \citeyearpar{brierloss}} & \textbf{DCA \citeyearpar{dcapaper}}   & \textbf{MMCE \citeyearpar{kumarpaper}} & \textbf{FLSD \citeyearpar{focallosspaper}}  & \textbf{FL+MDCA (ours)} \\ \midrule
                           & ResNet32       & 7.46                   & 7.67                & 7.52        & 7.76                & 7.06         & 8.41                    & 7.87              & 7.18    \\
\multirow{-2}{*}{CIFAR10}  & ResNet56       & 6.93                   & 7.26                & 6.43        & 7.75                & 6.53         & 8.23                    & 7.04              & 7.08     \\ \midrule
                           & ResNet32       & 31.29                  & 32.64               & 30.2        & 33.53               & 29.67        & 31.62                   & 32.15             & 31.58    \\
\multirow{-2}{*}{CIFAR100} & ResNet56       & 26.73                  & 28.67               & 26.49       & 30.72               & 43.43       & 28.75                   & 29.11             & 29.8       \\ \midrule
                           & ResNet20       & 3.86                   & 3.83                & 3.76        & 3.56                & 3.83         & 4.12                    & 4.10              & 3.92    \\
\multirow{-2}{*}{SVHN}     & ResNet56       & 3.60                   & 3.21                & 3.51        & 3.25                & 3.32         & 4.26                    & 3.65              & 3.85     \\ \midrule
Mendeley V2                & ResNet50       & 16.83                  & 17.63               & 17.15       & 18.43               & 17.47        &  15.06                  & 19.71                 & 17.95     \\ \midrule
Kather5000                 & ResNet34       & 16.90                  & 16.90               & 16.70       & 16.50               & 16.80        & 17.90                   & 19.30                 & 16.60   \\ \midrule
Tiny-ImageNet              & ResNet34       & 36.01                  & 37.48               & 35.73       & 43.00               & 36.68        & 40.75                   & 37.01             & 37.49              \\ \midrule
20 Newsgroups             & Global-Pool CNN       & 26.60                  & 28.80           & 27.78      & 25.93               & 28.07          & 28.63     &  30.80        & 27.88             \\ \bottomrule
\end{tabular}%
}

\caption{ Test Error (\%) values comparing various competing and our proposed method across various datasets and DNN architectures. Notice, near perfect calibration is achieved without sacrificing much on the DNN accuracy.}
\label{tab:testErr}
\end{table*}


% Merged SCE, ECE and 
\begin{table}[]
\centering
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc}
\toprule
\textbf{Domain}  & \textbf{NLL} & \textbf{NLL+MDCA} & \textbf{LS} & \textbf{LS+MDCA} & \textbf{FL} & \textbf{FL+MDCA} \\ 
\midrule
\multicolumn{7}{c}{\textbf{ECE (\%)}}\\
\midrule
Clean            & 0.11         & 0.22              & 9.89        & 9.83             & 1.34        & 0.79             \\
$M_{15}$         & 0.38         & 0.21              & 9.32        & 9.41             & 3.11        & 2.03             \\
$M_{30}$         & 1.13         & 1.31              & 7.13        & 7.38             & 3.92        & 2.94             \\
$M_{45}$         & 10.54        & 12.50             & 6.86        & 8.41             & 5.21        & 6.18             \\
$M_{60}$         & 31.95        & 35.02             & 27.36       & 25.32            & 28.11       & 25.77            \\
$M_{75}$         & 45.06        & 49.41             & 37.28       & 38.41            & 41.17       & 39.29            \\ \midrule
\textbf{Average} & 14.86        & 16.45             & 16.31       & 16.46            & 13.81       & 12.83 \\ 
\bottomrule  \\
\multicolumn{7}{c}{\textbf{Accuracy/Top-1 (\%)}}\\    
\midrule
Clean            & 99.61                            & 99.64                                  & 99.62                           & 99.63                                 & 99.63                           & 99.59                                \\
$M_{15}$         & 98.79                            & 98.63                                  & 98.39                           & 98.45                                 & 98.20                           & 98.61                                \\
$M_{30}$         & 93.38                            & 93.23                                  & 92.04                           & 92.54                                 & 91.87                           & 93.13                                \\
$M_{45}$         & 73.82                            & 71.53                                  & 69.33                           & 69.74                                 & 69.95                           & 70.92                                \\
$M_{60}$         & 43.24                            & 41.27                                  & 39.94                           & 41.88                                 & 38.67                           & 41.93                                \\
$M_{75}$         & 24.07                            & 22.05                                  & 22.99                           & 22.97                                 & 20.83                           & 23.37                                \\ \midrule
\textbf{Average} & 72.15                            & 71.06                                  & 70.39                           & 70.87                                 & 69.86                           & 71.26    \\ \bottomrule
\end{tabular}%
}
\caption{Ablation comparing ECE (\%) and Top-1 (\%) accuracy values of MDCA regularized losses with their unregularized versions on the Rotated-MNIST dataset trained on a ResNet-20 model.}
\label{tab:rot-mnist-ece-top1-ablation}
\end{table}


\begin{table}[]
\centering
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{c|ccc|c}
\toprule
\textbf{ECE (\%)}\\
\textbf{Methods}        & \textbf{Art} & \textbf{Cartoon} & \textbf{Sketch} & \textbf{Average} \\ \midrule
\textbf{Brier Score}    & 3.35         & 33.68            & 42.61           & 26.55            \\
\textbf{NLL}            & 9.42         & 52.99            & 35.56           & 32.66            \\
\textbf{LS}             & 8.70         & 25.21            & 13.29           & 15.73            \\
\textbf{Focal Loss}     & 7.34         & 48.96            & 25.33           & 27.21            \\
\textbf{MMCE}           & 17.06        & 43.25            & 40.79           & 33.70            \\
\textbf{DCA}            & 13.38        & 55.20            & 37.76           & 35.45            \\
\textbf{FLSD}           & 8.41         & 34.43            & 30.01           & 24.28            \\ \midrule
\textbf{FL+MDCA (ours)} & 6.29         & 29.81            & 23.05           & 19.71  \\ 
\bottomrule   
\textbf{Top-1(\%) accuracy}     \\
\bottomrule
 \textbf{Brier Score}    & 59.28        & 24.83            & 28.43           & 37.51            \\
\textbf{NLL}            & 59.08        & 21.20            & 28.00           & 36.09            \\
\textbf{LS}             & 56.35        & 22.01            & 29.88           & 36.08            \\
\textbf{Focal Loss}     & 52.83        & 17.32            & 26.70           & 32.28            \\
\textbf{MMCE}           & 60.60        & 29.95            & 20.36           & 36.97            \\
\textbf{DCA}            & 57.91        & 20.86            & 28.30           & 35.69            \\
\textbf{FLSD}           & 54.54        & 20.82            & 29.35           & 34.90            \\ \midrule
\textbf{FL+MDCA (ours)} & 63.23        & 27.86            & 23.01           & 38.03      \\ \bottomrule     
 
\end{tabular}%
}
\caption{Table comparing ECE and Accuracy (Top-1\%)  values of MDCA regularized losses with other methods on the PACS~\cite{pacspaper} trained on a ResNet-20 model and PACS dataset on ResNet 18 model.}
\label{tab:rmnist-pacs-ece-all_methods}
\end{table}


%\begin{enumerate}[leftmargin=*]
  	\item Additional results (See Sec. \ref{sec:addnlRes}) comprising of: (a) Class-j-ECE score to measure class-wise calibration - See Table \ref{tab:classECE_CIFAR10}; (b) For ablation study to understand the impact of various auxiliary losses such as DCA \cite{dcapaper}, \cite{kumarpaper} and ours with classification losses, namely, Label Smoothing(LS) \cite{labelsmoothinghelp}, Focal Loss \cite{focallosspaper} -- see Table \ref{tab:AblCIFARnSVHN} (c) Table \ref{tab:rot-MNIST} shows the study of MDCA
regularized losses with their unregularized versions.  we demonstrate the efficacy of our proposed on calibration performance using MDCA Aux. loss; (d) Table \ref{tab:rot-mnist-ece-top1-ablation} shows Accuracy/Top-1 (\%) values of
MDCA regularized losses with their unregularized versions, Here we show that our proposed loss \texttt{FL+MDCA} yields the best performance in case of Rotated MNIST dataset, (e) Table \ref{tab:rmnist-pacs-ece-top1-all_methods} shows results our method against others (top 1\% accuracy and ECE) on  dataset drift on PACS dataset\cite{pacspaper}. To conclusively understand the role of MDCA regulariser with auxilary losses refer to Table \ref{tab:ece-top1-rot-pacs-ablation}. We also report on Rotated MNIST\cite{can-u-trust} SCE scores in table \ref{tab:SCE-rot-MNIST} where we show MDCA regularised variants preserve calibration despite the dataset	drift. Again, to ablation on Rotated MNIST hint that our approach preserves calibration in dataset drift on Rotated MNIST dataset, refer to Table \ref{tab:rot-mnist-ece-top1-ablation} for details. Our proposed method \texttt{FL+MDCA} more or less preserves top-1 (\%) accuracy post-calibration as seen from Table \ref{tab:mnist-top1-all_methods}. Similarly, Table \ref{tab:SCE-rot-MNIST} compares the utility of MDCA regularisation in case of classification losses, NLL, LS and FL (f)  Test Error obtained after training with various competing methods and our proposed method (See Table \ref{tab:testErr})
 \end{enumerate}

% Abstract Aug 30, 2021

	Modern Deep Neural Networks are known to make  over-confident mistakes, which makes their use problematic in safety critical applications like self-driving vehicle, and healthcare. Contemporary calibration techniques consider the maximum confidence score of the predicted label alone. This leaves the confidence score of remaining non-max classes un-calibrated. Such a calibration has limited utility, since it can not be used to strengthen the decision making process, when a downstream task may want to switch the predicted label using prior or incorporating an auxiliary information. In this paper we argue for the calibration of the entire confidence vector, and use Static Calibration Error (SCE)~\cite{nixon2019measuring} to measure the same. In contrast to the contemporary post-hoc calibration approaches on a held-out dataset, we propose a learnable calibration technique, using a novel auxiliary loss function: \textbf{M}ulti-class \textbf{D}ifference in \textbf{C}onfidence and \textbf{A}ccuracy (MDCA), which can be used during the training stage in conjunction with other application specific loss functions. We show that training with MDCA leads to better calibrated models not only in terms of SCE, but also on the currently used Expected Calibration Error (ECE), which measures calibration for the predicted label only. We report ECE(SCE) score of \textbf{0.72(1.60)} on the CIFAR100 dataset, in comparison to 1.90(1.71) by the existing learnable calibration methods. Furthermore, we show that training with MDCA retains calibration reliably even under natural domain shift. For example, a ResNet-18 model trained on PACS dataset using MDCA gives a average ECE(SCE) score of \textbf{19.7(9.7)} across all domains, in comparison to a score of 24.2(11.8) by one of the recently proposed calibration methods. 


% The file aaai.sty is the style file for AAAI Press 
% proceedings, working notes, and technical reports.


Many modern Deep Neural Networks (DNNs) are found to be poorly calibrated i.e., the DNN output accuracies often do not perfectly align with the predicted probabilities posing reliability concerns in safety critical pipelines. The existing works calibrate the predicted confidence score of DNNs, without taking into account the underlying class-wise probability distribution in a multi-class classification setting ignoring calibration for classes other than the predicted class with highest confidence This moreover overlooks a fundamental principle that probabilities are much more informative than a label.
%~\cite{guo2017calibration, ecepaper, kumarpaper}.
\textcolor{red}{The calibration of predictive probability vector is particularly important as (a)  we desire the models to be calibrated across all
predictions when no true class label is likely in case of label noise \cite{nixon2019measuring} or data noise (natural corruptions); (b) a study conducted by \cite{tsoukalas2015data} concluded in physicians/radiologists caring about a secondary or tertiary prediction also as the incorrect decision lead to monetary and ethical implications necessitating a comprehensive view of the likelihoods of all potential outcomes; and (c) post-calibration is anticipated to result in optimal usage of human intervention as predictive probabilities are closer to actual outcomes}. In light of this, we make following contributions : (a) a trainable approach to calibrate DNNs utilising our proposed auxiliary loss, \textbf{M}ulti-class \textbf{D}ifference in \textbf{C}onfidence and \textbf{A}ccuracy (\textbf{MDCA}); (b) We demonstrate that MDCA functions as a powerful regularizer when combined with any classification loss such as the cross entropy, label smoothing, and focal loss to boost calibration performance; (c) Our exhaustive experiments demonstrate that training with MDCA and focal loss improves probabilistic predictions according to well-known calibration measures. We provide competitive performance among trainable methods across wide range of benchmark datasets. Finally, performance of our approach in combination with post-hoc calibration furthers predictive uncertainty at the same time preserving calibration on dataset drift on standard datasets.
% instead just mentioning that in case of medical field , physician may care about some top-few predictions is enough for multiclass calibration

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc|ccc}
\toprule
\textbf{Dataset}          & \textbf{Model} & \textbf{Cross Entropy} & \textbf{Focal Loss} & \textbf{LS} & \textbf{Brier Loss} & \textbf{DCA} & \textbf{MMCE} & \textbf{LS+MDCA (ours)} & \textbf{NLL+MDCA (ours)}  & \textbf{FL+MDCA (ours)}  \\ \midrule
\multirow{2}{*}{CIFAR10}  & ResNet34       & 3.99                   & 4.60                & 6.13        & 4.37                & 3.61         & 9.25          & 6.76                    & 3.71                  & -   \\
                           & ResNet56       & 3.25                   & 3.91                & 4.49        & 3.93                & 3.00         & 5.56          & 5.65                    & 3.23               & -      \\ \midrule
 \multirow{2}{*}{CIFAR100} & ResNet34       & 1.56                   & 1.81                & 1.91        & 1.77                & 1.57         &               & 1.65                    & 1.58   
\begin{table}[]
\centering
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{c|ccc|c}
\toprule
\textbf{ECE (\%)}\\
\textbf{Methods}        & \textbf{Art} & \textbf{Cartoon} & \textbf{Sketch} & \textbf{Average} \\ \midrule
\textbf{Brier Score}    & 3.35         & 33.68            & 42.61           & 26.55            \\
\textbf{NLL}            & 9.42         & 52.99            & 35.56           & 32.66            \\
\textbf{LS}             & 8.70         & 25.21            & 13.29           & 15.73            \\
\textbf{Focal Loss}     & 7.34         & 48.96            & 25.33           & 27.21            \\
\textbf{MMCE}           & 17.06        & 43.25            & 40.79           & 33.70            \\
\textbf{DCA}            & 13.38        & 55.20            & 37.76           & 35.45            \\
\textbf{FLSD}           & 8.41         & 34.43            & 30.01           & 24.28            \\ \midrule
\textbf{FL+MDCA (ours)} & 6.29         & 29.81            & 23.05           & 19.71  \\ 
\bottomrule   
\textbf{Top-1(\%) accuracy}     \\
\bottomrule
 \textbf{Brier Score}    & 59.28        & 24.83            & 28.43           & 37.51            \\
\textbf{NLL}            & 59.08        & 21.20            & 28.00           & 36.09            \\
\textbf{LS}             & 56.35        & 22.01            & 29.88           & 36.08            \\
\textbf{Focal Loss}     & 52.83        & 17.32            & 26.70           & 32.28            \\
\textbf{MMCE}           & 60.60        & 29.95            & 20.36           & 36.97            \\
\textbf{DCA}            & 57.91        & 20.86            & 28.30           & 35.69            \\
\textbf{FLSD}           & 54.54        & 20.82            & 29.35           & 34.90            \\ \midrule
\textbf{FL+MDCA (ours)} & 63.23        & 27.86            & 23.01           & 38.03      \\ \bottomrule     
 
\end{tabular}%
}
\caption{Table comparing ECE and Accuracy (Top-1\%)  values of MDCA regularized losses with other methods on the PACS~\cite{pacspaper} trained on a ResNet-20 model and PACS dataset on ResNet 18 model.}
\label{tab:rmnist-pacs-ece-all_methods}
\end{table}            & -      \\
                           & ResNet56       & 1.49                   & 1.62                & 1.67        & 1.68                & 1.56         &               & 1.80                    & 1.55               & -      \\ \midrule
 \multirow{2}{*}{SVHN}     & ResNet20       & 2.72                   & 3.03                & 5.57        & 2.45                & 2.17         & 8.89          & 3.36                    & 2.94                & -     \\
                           & ResNet56       & 4.15                   & 2.71                & 3.11        & 2.18                & 3.09         & 7.35          & 1.77                    & 3.45              & -       \\ \midrule
 Mendeley V2                  & ResNet50       & 147.7                  & 143.8               & 139.8       & 164.3               & 155.7        &               & 89.5                    & 40.7           & -          \\ \midrule
 Kather5000                & ResNet34       & 26.34                  & 27.44               & 25.86       & 25.59               & 28.34        & 27.83         & 29.32                   & 26.46                & -    \\ \bottomrule
 \end{tabular}%
 }
\caption{ SCE (to the scale of $10^{-3}$) values (with $M=15$ bins) comparing various baselines and our proposed methods \textbf{after performing Temperature scaling as post-hoc calibration\ramya{this does not have TS results: Wanted to see pre and post TS, similarly Direchlet }}}
\label{tab:sce_posthoc}
\end{table*}



% well trained deep classifiers are often overconfident even for novel examples, unseen during training

\paragraph{Optimising hyper-parameter $\beta$}: For details on how hyper-parameter $\beta$ refer supplemental material. Figure \ref{fig:EffectofbetaOnSCE}) shows a trend that calibration is best achieved when $\beta$ is close to 1, and as we increase it, accuracy decreases and the SCE score increases.

% From data to optimal decision making: a data-driven, probabilistic machine learning approach to decision support for patients with sepsis:  our ability to efficiently extract informed decision support is limited due to the complexity of the clinical states and decision process, missing data and lack of analytical tools to advice based on statistical relationships. Objective: Development and assessment of a data-driven method that infers the probability distribution of the current state of patients with sepsis, likely trajectories, optimal actions related to antibiotic administration, prediction of mortality and length-of-stay.

%Multi-class and discriminative classifiers were used to predict mortality and length of stay.

% A data-driven model was able to suggest favorable actions, predict mortality and length of stay with high accuracy. This work provides a solid basis for a scalable probabilistic clinical decision support framework for sepsis treatment that can be expanded to other clinically relevant states and actions, as well as a data-driven model that can be adopted in other clinical areas with sufficient training data.

% Over the past few decades, our society has transitioned to a state where bottlenecks have shifted from a lack of data, to limitations in extracting meaningful knowledge and subsequently use that knowledge to drive decisions. This data-rich, knowledge-poor oxymoron is particularly true in computationally-driven Clinical Decision Support Systems (CDSS), where advances in automated high-throughput data acquisition and electronic health records have yet to be translated into knowledge extraction and probabilistic decision guidance. This is true even in the cases of dangerous and ubiquitous threats to human health, one of which is sepsis. Sepsis is an overwhelming systemic immune response to infection, which results in damage to the patients’ own tissues and organs. This process can happen at any age, regardless of the underlying health condition and from seemingly benign incidents. Severe sepsis strikes about 18 million people annually (750,000 cases in the United States) and has a very high short-term mortality risk (28% to 50%) [1] Severe sepsis is the leading cause of Intensive Care Unit (ICU) deaths (60-80% of ICU deaths in developing countries) and it kills more than 6 million children world-wide every year [2].


%  To this end, we propose an effective calibration technique for image classifiers, where DNN predictions model the  predictive uncertainty score to the real world predictions as closely as possible.


% They focus on minimising Expected Calibration Error (ECE), rather than Static Calibration Error (SCE) which is more appropriate in a multi-class setting. 

% NOTE: we have not compared against all trainable methods, so we cannot claim state of the art.



This are some references and keywords that are descriptive of calibration

\begin{itemize}
{ 
%\item \textbf{Temperature Scaling}: It is a modern variant of Platt scaling, that works by dividing the logits by a scalar $T > 0$ (which is learnt on a hold-out training set), prior to taking a softmax, $\sigma_{SM}(z_{i}))^{k} = \frac{\exp(z^{(k)}_{i})}{\sum_{j = 1}^{K} \exp(z^{(k)}_{i}$
%It is the most common approach to calibrate DNNs. Its easy, fast and performs well usually. Temperature scaling has the desirable property that it improve calibration without affecting the accuracy. However, it has it's downsides too. Temperature Scaling reduces the confidence of every prediction, even the correct ones [sunita maams paper]. Being a post-proccessing step, it does not help in feature learning [DCA paper]. It also does not calibrate a model under data distribution shift [Can You Trust Your Model’s Uncertainty paper].

%\item \textbf{Matrix Scaling\parencite{}}: A more general version of temperature scaling, wherein instead of dividing the logits by a single scalar, we multiply it by a matrix $M$. We learn the matrix $M$ on the hold-out set similar to temprature scaling.

\item \textbf{Dirichlet Calibration [\parencite{kull2019beyond}]}: This method takes a prior of the form of a multivariate $\beta$-distribution into account when calibrating. \parencite{kull2019beyond} assume that $\hat{p}(X) | (Y=j) \sim $ Dirichlet$(\alpha^{(j)})$, where $\alpha^{(j)} \in \mathbb{R}^K$. Dirichlet calibration is easy to implement as an extra layer in a neural net, or as multinomial logistic regression on log-transformed class probabilities, learnt on the hold-out set. Kull et al. also propose a new regularisation method called \textbf{ODIR} or Off-Diagonal regularisation, defined as   $ODIR = \frac{1}{k*(k-1)}\sum_{i \neq j}w_{i,j}^2$
}}
\end{itemize}




%\item \textbf{Label Smoothing}: Muller et al. proposed that training on soft-targets helps in improving calibration implicitly as well as clustering of individual classes. 
\begin{equation}
    LS = - \sum_{i=1}^N \sum_{j=1}^K q_{i,j} \log (\hat{p}_{i,j})
\end{equation}
where \textbf{${q_{i}}$} are the soft-targets defined as $q_{i,j}=\alpha/(K-1)$ if $j \neq y_i$ else $q_{i,j} = (1-\alpha)$, here $\alpha$ is a hyper-parameter.



\section{Why learn-able calibration is appealing ?}
\begin{itemize}
    \item No extra hold out set is required
    \item post-hoc calibration does not do feature learning [cite liang et al]
    \item A DNN should be able to calibrate itself without any post-processing
\end{itemize}





%\neels{on the metrics to measure calibration and the methods to reduce miscalibration}. Given the importance of calibration, various metrics have been developed to measure the degree of miscalibration (Section 2.1). There have been multiple attempts at solving the problem of miscalibration, of which most can be divided into sub categories of Trainable Calibration Methods (Section 2.2) and Post-Hoc Calibration Methods (Section 2.3)

%\neels{we cannot write too much about why misclassification as it takes direct inspiration form the paper, if we have to then we shall require some extra insight}

%\neels{100\% calibraiton but 0\% accuracy} %It is very common for classifiers to be trained using a Negative-Log-Liklihood (NLL) loss. However, there is an inherent bug within the NLL Loss. Although NLL can be used to indirectly optimize for calibration, models trained with NLL tend to be over-confident\neels{Enter citation}. During training, the authors observe a disconnect between NLL and accuracy, paves way for justifying the overconfident scores and hence the  miscalibration.

Overfitting the loss but not the accuracy Note that the NLL is minimised when for each training sample $i$, $\hat{p}_{i,y_i} = 1$, whereas the classification error is minimised when $\hat{p}_{i,y_i} > \hat{p}_{i,y}$ for all $y \neq y_i$. This means that even when the classification error is 0, the NLL can be positive, and the optimisation algorithm can still try to reduce it to 0 by further increasing the value of $\hat{p}_{i,y_i}$ for each sample $i$. This is the reason for overfitting and over-confidence.


Why Miscalibration happens in the first place ?
define NLL and issues with NLL, Depth of Neural network, width, weight decay

\neels{ \textbf{Inherent bug in NLL loss}: 
Overfitting the loss but not the accuracy Note that the NLL is minimised when for each training sample $i$, $\hat{p}_{i,y_i} = 1$, whereas the classification error is minimised when $\hat{p}_{i,y_i} > \hat{p}_{i,y}$ for all $y \neq y_i$. This means that even when the classification error is 0, the NLL can be positive, and the optimisation algorithm can still try to reduce it to 0 by further increasing the value of $\hat{p}_{i,y_i}$ for each sample $i$. This is the reason for overfitting and over-confidence.}
Why Miscalibration happens in the first place ?
define NLL and issues with NLL, Depth of Neural network, width, weight decay

cluster the calibration methods \\


\ramya{we consider a set of $N$ training samples, $\D_\text{in}^\text{train} = (x_n, y_n)^N_{n=1}$, where $\D_\text{in}^\text{train}$ is drawn independently from a probability distribution: $\cP_{X,Y}$. Here, $X\in\X$ is a random variable defined on the image space, and $Y\in\Y = \{1,\ldots,K\}$ is a random variable representing its label. A classifier $f_{\theta}:\mathcal{X} \rightarrow \mathcal{Y}$ is trained on the in-distribution samples drawn from the marginal distribution $\cP_X$ of $X$ derived from the joint distribution $\cP_{X,Y}$. Here $\theta$ refers to model parameters learnt by the neural network.}

Modern Deep Neural Networks (DNNs) are often miscalibrated i.e., they make overconfident/underconfident decisions. The DNN accuracies often do not perfectly align with the predicted probabilities posing reliability concerns for decision making in safety critical pipelines. To this end, we propose an effective calibration technique for image classifiers with the aim where DNN predictions model the real world as closely as possible i.e., the confidence scores reflect the true probability distributions of the outputs and provide an interpret-able meaning to a confidence score. Many existing works calibrate the predicted confidence score of DNNs, without taking into account the underlying class-wise probability distribution in a multi-class classification setting. This ignores calibration for classes other than the than the predicted class with highest confidence which could possibly be incorrect. Such approaches focus on minimising Expected Calibration Error (ECE), rather than Static Calibration Error more suitable in a multi-class setting. To address this, we propose a trainable approach to calibrate DNNs utilising a novel differentiable auxiliary loss, \textbf{M}ulti-class \textbf{D}ifference in \textbf{C}onfidence and \textbf{A}ccuracy (\textbf{MDCA}) which could be clubbed with any loss terms such as the cross entropy, label smoothing, Direchlet calibration. We demonstrate MDCA promotes calibration over the recent state-of-the-art trainable methods on standard benchmark datasets and performs on-par with the post-hoc calibration techniques.



Gneiting, T., Balabdaoui, F., and Raftery, A. E. Probabilistic forecasts, calibration and sharpness.
Journal of the Royal Statistical Society, 2007

ECE -- source: Naeini, M. P., Cooper, G., and Hauskrecht, M. Obtaining well calibrated probabilities using bayesian
binning. In AAAI Conference on Artificial Intelligence, 2015.

conformal prediction : Shafer, G. and Vovk, V. A tutorial on conformal prediction. Journal of Machine Learning Research,
2008.

DeGroot, M. H. and Fienberg, S. E. The comparison and evaluation of forecasters. Journal of the
Royal Statistical Society, 1983.

accuracy under distribution shift

. The important implication of
this result is that designing models based on in-distribution performance likely also benefits their
out-of-distribution performance

too certain (overconfident), optimally confident, or too
uncertain (underconfident)

Michael W. Dusenberry, Dustin Tran, Edward Choi, Jonas Kemp, Jeremy Nixon, Ghassen Jerfel,
Katherine Heller, and Andrew M. Dai. Analyzing the role of model uncertainty for electronic
health records. In Proc. of the ACM Conference on Health, Inference, and Learning (ACM
CHIL), pp. 204–213, Toronto Ontario Canada, April 2020. ACM. ISBN 978-1-4503-7046-2. doi:
10.1145/3368555.3384457. URL http://arxiv.org/abs/1906.03842

% Confidence calibration
Kimin Lee, Honglak Lee, Kibok Lee, and Jinwoo Shin. Training confidence-calibrated classifiers for
detecting out-of-distribution samples. arXiv preprint arXiv:1711.09325, 2017.

% extending calibration in regression
Volodymyr Kuleshov, Nathan Fenner, and Stefano Ermon. Accurate uncertainties for deep learning
using calibrated regression. arXiv preprint arXiv:1807.00263, 2018.

% calibration: Pathologies with just taking argmax

We examine increasing the importance of omitted predictions via label noise. As label noise increases,
trained models become less confident in their predictions. Secondary and tertiary predictions are
correct with higher frequency, and so for many samples the prediction with the correct label isn’t
included in ECE’s measure of calibration error. We find that ECE becomes a worse approximation of
the calibration error as relevant predictions not included in the ECE metric become common (Figure
1).

% need for secondary and teritiary predictions

Athanasios Tsoukalas, Timothy Albertson, and Ilias Tagkopoulos. From Data to Optimal Decision
Making: A Data-Driven, Probabilistic Machine Learning Approach to Decision Support for
Patients With Sepsis. JMIR Medical Informatics, 3(1):e11, February 2015. ISSN 2291-9694. doi:
10.2196/medinform.3445. URL http://medinform.jmir.org/2015/1/e11/.


% Aug 21, 2021

% Ondrej Bohdal, Yongxin Yang and Timothy Hospedales. Meta-Calibration: Meta-Learning of Model Calibration Using Differentiable Expected Calibration Error

accurate estimates

Meta learning for calibration

 simple posttraining rescaling of the logits – temperature scaling – works
relatively well. Kumar et al. (2018) propose a kernel-based
measure of calibration that they use as regularization during
training of neural networks. Mukhoti et al. (2020) show
focal loss – a relatively simple weighted alternative to crossentropy – can be used to train well-calibrated neural networks. The classic Brier score (Brier, 1950), which is the
squared error between the softmax vector with probabilities and the ground-truth one-hot encoding, has also been
show to work well. Similarly, label smoothing (Muller et al. ¨ ,
2019) has also been shown to improve model calibration

This is an efficient strategy as we do not need to
backpropagate through many inner-loop steps or retrain the
model from scratch for each update of meta-knowledge

%  Class-Distribution-Aware Calibration for Long-Tailed Visual Recognition - ICML Workshop

 Recent techniques like temperature scaling (TS) and label smoothing (LS)
show effectiveness in obtaining a well-calibrated
model by smoothing logits and hard labels with
scalar factors, respectively. However, the use of
uniform TS or LS factor may not be optimal for
calibrating models trained on a long-tailed dataset
where the model produces overly confident probabilities for high-frequency classes.


% Jishnu Mukhoti - Focal loss 

negative log-likelihood loss, they overfit
to datasets, rendering its predictions to be over-confident and
less trustworthy (Mukhoti et al., 2020).

% M. To
find the optimal temperature, a conjugate gradient solver or
a naive line-search is used on a trained model without affecting model accuracy (


% post hoc calibration table with all resnets
\begin{table}[]
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
  \multirow{2}{*}{\textbf{Post Hoc}} &
  \multicolumn{2}{c}{\textbf{CIFAR10}} &
  \multicolumn{2}{c}{\textbf{CIFAR100}} &
  \multicolumn{2}{c}{\textbf{SVHN}} \\
 &
   &
  \textbf{RN34} &
  \textbf{RN56} &
  \textbf{RN34} &
  \textbf{RN56} &
  \textbf{RN20} &
  \textbf{RN56} \\ \midrule
\multirow{3}{*}{Brier}   & None & 6.61  & 5.44  & 1.97 & 1.86 & 2.46  & 2.18  \\
                         & TS    & 4.37  & 3.94  & 1.78 & 1.68 & 2.46  & 3.88  \\
                         & DC & 3.89  & 4.83  & 1.89 & 1.80 & 1.91  & 2.11  \\ \midrule
\multirow{3}{*}{NLL}     & None & 8.68  & 7.12  & 2.40 & 2.50 & 3.43  & 3.84  \\
                         & TS    & 3.99  & 3.25  & 1.56 & 1.49 & 4.13  & 4.16  \\
                         & DC & 3.07  & 4.98  & 2.17 & 1.91 & 2.48  & 2.69  \\ \midrule
\multirow{3}{*}{LS}      & None & 14.09 & 12.55 & 1.99 & 1.73 & 18.80 & 21.08 \\
                         & TS    & 6.13  & 4.49  & 1.91 & 1.67 & 2.35  & 3.12  \\
                         & DC & 5.96  & 5.34  & 2.05 & 1.98 & 2.36  & 2.81  \\ \midrule
\multirow{3}{*}{FL}      & None & 4.61  & 4.19  & 1.83 & 1.89 & 3.04  & 7.85  \\
                         & TS    & 3.77  & 4.19  & 1.82 & 1.62 & 3.04  & 2.72  \\
                         & DC & 4.69  & 5.48  & 2.02 & 2.02 & 2.28  & 3.36  \\ \midrule
\multirow{3}{*}{MMCE}    & None & 8.17  & 9.12  & 2.34 & 2.35 & 9.18  & 9.69  \\
                         & TS    & 4.68  & 4.05  & 1.56 & 1.61 & 5.01  & 3.74  \\
                         & DC & 8.10  & 6.26  & 2.02 & 1.95 & 4.70  & 5.11  \\ \midrule
\multirow{3}{*}{DCA}     & None & 8.41  & 7.60  & 2.82 & 2.87 & 4.29  & 2.16  \\
                         & TS    & 3.44  & 3.00  & 1.58 & 1.56 & 2.18  & 4.29  \\
                         & DC & 4.39  & 4.20  & 2.18 & 2.06 & 2.21  & 2.95  \\ \midrule
\multirow{3}{*}{FLSD}    & None & 9.49  & 7.71  & 1.77 & 1.71 & 18.98 & 26.15 \\
                         & TS    & 4.05  & 3.27  & 1.77 & 1.71 & 3.75  & 4.41  \\
                         & DC & 5.51  & 5.62  & 2.06 & 2.01 & 3.50  & 4.31  \\ \midrule
                         \rowcolor{LightCyan}
\multirow{3}{*}{FL+MDCA} & None & \textbf{3.22}  & \textbf{2.93}  & \textbf{1.72} & \textbf{1.60} & \textbf{1.90}  & \textbf{1.51} \\
                         & TS    & 3.24  & 2.93  & 1.77 & 1.60 & 1.90  & 5.00  \\
                         & DC & 5.33  & 3.81  & 2.07 & 1.87 & 2.38  & 2.72  \\ \bottomrule
\end{tabular}%
}
\caption{Ablatuon of trainable methods with Post-Hoc Calibration. Observe that our proposed method reports the least SCE(\%) in comparison to any trainable.Post Hoc method. Note TS: Temperate scaling~\cite{platt1999probabilistic}; DC: Dirichlet Calibration~\cite{Dirichlet}}
\label{tab:TrainVsPH}
\end{table}


% SCE scores all methods
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc|c}
\toprule
\textbf{Dataset}          & \textbf{Model} & \textbf{Cross Entropy} & \textbf{Focal Loss \citeyearpar{ogfocalloss}} & \textbf{LS \citeyearpar{labelsmoothinghelp}} & \textbf{Brier Score \citeyearpar{brierloss}} & \textbf{DCA \citeyearpar{dcapaper}}   & \textbf{MMCE \citeyearpar{kumarpaper}} & \textbf{FLSD \citeyearpar{focallosspaper}}  & \textbf{FL+MDCA (ours)} \\ \midrule
\multirow{2}{*}{CIFAR10}  & ResNet34       & 8.68                  & 4.60           & 14.08     & 6.60               & 8.41          & 8.17     & 9.48         & \textbf{3.22}                    \\
                          & ResNet56       & 7.11                  & 4.18           & 12.54     & 5.44               & 7.59          & 9.11     & 7.71         & \textbf{2.93}                \\ \midrule
\multirow{2}{*}{CIFAR100} & ResNet34       & 3.03                  & 1.83           & 1.99      & 1.97               & 2.82          & 2.79     & 1.77         & \textbf{1.72}                  \\
                          & ResNet56       & 2.50                  & 1.66           & 1.73      & 1.86               & 2.77          & 2.35     & 1.71         & \textbf{1.60}              \\ \midrule
\multirow{2}{*}{SVHN}     & ResNet20       & 3.43                  & 2.54           & 18.80     & 2.12               & 4.29          & 9.18     & 18.98        & \textbf{1.90}          \\
                          & ResNet56       & 3.84                  & 7.85           & 21.08     & 2.18               & 2.16          & 9.69     & 26.15        & \textbf{1.51}        \\ \midrule
Mendeley V2               & ResNet50       & 131.2                 & 108.3          & 103.8     & 117.6              & 145.1         & 130.4    &  104.3           & \textbf{85.68}         \\ \midrule
Kather5000                & ResNet34       & 31.70                 & 41.69          & 46.63     & 32.76              & \textbf{27.13} & 47.35   &  57.87           & 41.39              \\ \midrule
Tiny-ImageNet             & ResNet34       & 1.91                  & 1.19           & 1.38      & 1.53               & 2.11          & 1.62     &  1.18        & \textbf{1.17 }             \\ \midrule
20 Newsgroups             & Global-Pool CNN       & 602.68                  & 729.39           & 988.42      & 725.82               & 719.83          & 731.31     &  940.70        & \textbf{487.82 }             \\ \bottomrule
\end{tabular}%
}
\caption{ SCE (to the scale of $10^{-3}$) values (with $M=15$ bins) comparing various competing methods and our proposed method across well-known classification benckmarks and DNN architectures. We outperform all the baselines except in some occasions where our method yields comparable score to best performing one.}
\label{tab:sce-m15}
\end{table*}

% ECE % scores all methods
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc|c}
\toprule
\textbf{Dataset}          & \textbf{Model} & \textbf{Cross Entropy} & \textbf{Focal Loss \citeyearpar{ogfocalloss}} & \textbf{LS \citeyearpar{labelsmoothinghelp}} & \textbf{Brier Score \citeyearpar{brierloss}} & \textbf{DCA \citeyearpar{dcapaper}}   & \textbf{MMCE \citeyearpar{kumarpaper}} & \textbf{FLSD \citeyearpar{focallosspaper}}  & \textbf{FL+MDCA (ours)} \\ \midrule
\multirow{2}{*}{CIFAR10}  & ResNet34       & 4.25                   & 1.76       & 6.28             & 2.92                & 4.00          & 3.31          & 4.41          & \textbf{0.93}     \\
                          & ResNet56       & 3.27                   & 1.11       & 5.38             & 2.17                & 3.38          & 3.71          & 3.49           & \textbf{0.70}          \\ \midrule
\multirow{2}{*}{CIFAR100} & ResNet34       & 12.45                  & 1.62       & 2.09             & 5.32                & 11.31         & 11.09         & 1.69           & \textbf{1.49}    \\
                          & ResNet56       & 9.32                   & 2.29       & 8.94             & 4.69                & 9.29          & 8.61          & 1.90           & \textbf{0.72}          \\ \midrule
\multirow{2}{*}{SVHN}     & ResNet20       & 1.64                   & 0.89       & 8.88             & \textbf{0.45}       & 2.02          & 4.34          & 9.37           & 0.47       \\
                          & ResNet56       & 1.82                   & 3.89       & 10.00            & 0.66                & 0.49          & 4.48          & 13.23           & \textbf{0.23}          \\ \midrule
Mendeley V2               & ResNet50       & 4.78                   & 8.17       & \textbf{2.68}    & 3.75                & 8.29          & 3.45             & 9.64           & 4.81        \\ \midrule
Kather5000                & ResNet34       & 7.14                   & 13.62      & 15.36            & 8.64                & \textbf{4.49} & 16.63         & 22.03           & 13.45   \\ \midrule
Tiny-ImageNet             & ResNet34       & 14.91                  & 2.26       & 5.96             & 7.79                & 17.40         & 9.71          & \textbf{1.91}           & 1.99              \\ \midrule
20 Newsgroups             & Global-Pool CNN       & 14.78                  & 13.35           & \textbf{3.45}      & 13.71               & 15.30          & 12.69     &  4.52        & 16.55             \\ \bottomrule
\end{tabular}%
}
\caption{ ECE (\%) values ($M=15$ bins) comparing competing and our method across various datasets and DNN architectures.}
\label{tab:ece-m15}
\end{table*}

% SCE / ECE scores all methods
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc|c}
\toprule
\textbf{Dataset}          & \textbf{Model} & \textbf{NLL} & \textbf{FL} & \textbf{LS} & \textbf{Brier Score} & \textbf{DCA}   & \textbf{MMCE} & \textbf{FLSD}  & \textbf{Ours} \\
 &  & & \citeyearpar{ogfocalloss} & \citeyearpar{labelsmoothinghelp} & \citeyearpar{brierloss} & \citeyearpar{dcapaper}   & \citeyearpar{kumarpaper} & \citeyearpar{focallosspaper}  &  \\
\midrule
\multirow{2}{*}{CIFAR10}  & ResNet32     &  8.68 / 4.25 &  4.60 / 1.76 &  14.08 / 6.28 &  6.60 / 2.92 &  8.41 / 4.00 &  8.17 / 3.31 &  9.48 / 4.41 &  3.22 / 0.93 \\
                          & ResNet56       & 7.11 / 3.27 &  4.18 / 1.11 &  12.54 / 5.38 &  5.44 / 2.17 &  7.59 / 3.38 &  9.11 / 3.71 &  7.71 / 3.49 &  2.93 / 0.70                \\ \midrule
\multirow{2}{*}{CIFAR100} & ResNet32       & 3.03 / 12.45 &  1.83 / 1.62 &  1.99 / 2.09 &  1.97 / 5.32 &  2.82 / 11.31 &  2.79 / 11.09 &  1.77 / 1.69 &  1.72 / 1.49         \\
                          & ResNet56       & 2.50 / 9.32 &  1.66 / 2.29 &  1.73 / 8.94 &  1.86 / 4.69 &  2.77 / 9.29 &  2.35 / 8.61 &  1.71 / 1.90 &  1.60 / 0.72     \\ \midrule
\multirow{2}{*}{SVHN}     & ResNet20       & 3.43 / 1.64 &  2.54 / 0.89 &  18.80 / 8.88 &  2.12 / 0.45 &  4.29 / 2.02 &  9.18 / 4.34 &  18.98 / 9.37 &  1.90 / 0.47       \\
                          & ResNet56    &  3.84 / 1.82 &  7.85 / 3.89 &  21.08 / 10.00 &  2.18 / 0.66 &  2.16 / 0.49 &  9.69 / 4.48 &  26.15 / 13.23 &  1.51 / 0.23        \\ \midrule
Mendeley V2               & ResNet50       & 131.2 / 4.78 &  108.3 / 8.17 &  103.8 / 2.68 &  117.6 / 3.75 &  145.1 / 8.29 &  130.4 / 3.45 &  104.3 / 9.64 &  85.68 / 4.81     \\ \midrule
Kather5000                & ResNet34       & 31.70 / 7.14 &  41.69 / 13.62 &  46.63 / 15.36 &  32.76 / 8.64 &  27.13 / 4.49 &  47.35 / 16.63 &  57.87 / 22.03 &  41.39 / 13.45              \\ \midrule
Tiny-ImageNet             & ResNet34       & 1.91 / 14.91 &  1.19 / 2.26 &  1.38 / 5.96 &  1.53 / 7.79 &  2.11 / 17.40 &  1.62 / 9.71 &  1.18 / 1.91 &  1.17 / 1.99            \\ \midrule
20 Newsgroups             & Global-Pool CNN       & 602.68 / 14.78 &  729.39 / 13.35 &  988.42 / 3.45 &  725.82 / 13.71 &  719.83 / 15.30 &  731.31 / 12.69 &  940.70 / 4.52 &  487.82 / 16.55         \\ \bottomrule
\end{tabular}%
}
\caption{ SCE (to the scale of $10^{-3}$) / ECE(\%) values (with $M=15$ bins) comparing various competing methods and our proposed method across well-known classification benckmarks and DNN architectures. We outperform all the baselines except in some occasions where our method yields comparable score to best performing one.}
\label{tab:sce-m15}
\end{table*}

==> sections/discussion.tex <==
\subsection{Discussion}
\label{subsec:disc}

Using a train-time calibration method helps in achieving  well-calibrated models, and with a post-hoc calibration method we demonstrate how calibration results can be enhanced. It is derirable to calibrate DNN at train-time procedure to reduce the reliance of a hold-out set to finetune the calibration measures. We have seen through above results that $\mathcal{L}_{MDCA}$ helps in doing so. In particular, our approach is promising and is more practical in low data regime without the luxury of access to a validation set, making our approach deployment friendly except for the minor cost born for retraining procedure. \textcolor{red}{Needs cross verification: the reason why FL + MDCA works well in class imbalance is because FL pays attention to classes with low label distribution/minority classes and also MDCA gives more weightage to minority classes} %Finally, with regards to deployment, it is harder to obtain a dataset for fine-tuning. 
Further, from our exhaustive ablation study when we try various off-the-shelf classification losses ($\mathcal{L}_C$) paired with the competing calibration inducing regularizer \cite{dcapaper, kumarpaper} and then with MDCA. Table  \ref{tab:sce-m15} shows regardless of what $\mathcal{L}_C$ is, we get consistently least SCE and ECE values with minor or no dip in accuracy. %In future, we would like to metalearn $\beta$, scalar for regularising Eqn. \ref{equ:totalLoss} to obtain the best possible calibration error automatically.



%\begin{itemize}
 %   \item Write the rationale for hybrid approaches
 %   \item Note on comaprison of trainable methods
 %   \item Note on camparison of post-hoc calibration methods and issues of access to validation dataset
  %  \item Note on inference time of all the methods
%\end{itemize}
